Compressing Large-Scale Transformer-Based Models: A Case Study on BERT

Pre-trained Transformer-based models have achieved state-of-the-art performance for various Natural Language Processing (NLP) tasks. However, these models often have billions of parameters, and, thus, are too resource-hungry and computation-intensive to suit low-capability devices or applications with strict latency requirements. One potential remedy for this is model compression, which has attracted a lot of research attention. Here, we summarize the research in compressing Transformers, focusing on the especially popular BERT model. In particular, we survey the state of the art in compression for BERT, we clarify the current best practices for compressing large-scale Transformer models, and we provide insights into the workings of various methods. Our categorization and analysis also shed light on promising future research directions for achieving lightweight, accurate, and generic NLP models.

==> tables/aaai_table.tex <==
\begin{table*}[!h]
\footnotesize
\centering
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\Xhline{3\arrayrulewidth}
 \textbf{Methods} & \textbf{Provenance} & \textbf{Target} & \multicolumn{2}{|c|}{\textbf{Model Size (MB)}} & \multicolumn{2}{|c|}{\textbf{Speedup}} & \multicolumn{4}{|c|}{\textbf{Accuracy/F1}} & \textbf{Avr.} \\
\cline{4-11}
 & & \textbf{Device} & \textbf{w/ emb} & \textbf{w/o emb} & \textbf{GPU} & \textbf{CPU} & \textbf{MNLI} & \textbf{QQP} & \textbf{SST-2} & \textbf{SQD} & \textbf{Drop} \\
\Xhline{3\arrayrulewidth}

$\mathrm{BERT}_{\mathrm{BASE}}$ & \cite{devlin2019bert} & -- & 420 (100\%) & 330 (100\%) & 1x & 1x & 84.6 & 89.2 & 93.5 & 88.5 & 0.0 \\
\Xhline{3\arrayrulewidth}

\multirow{2}{*}{Quantization} & \cite{shen2019q} $^{S}$ & -- & 63 (15\%) & 41 (12.5\%) & 1x & 1x & 83.9 & -- & 92.6 & 88.3 & -0.6 \\
\cline{2-12}
 & \cite{zadeh2020gobo} $^{S}$ & -- & 43 (10.2\%) & 18 (5.5\%) & 1x & 1x & 83.7 & -- & -- & -- & -0.9 \\
% \Xhline{3\arrayrulewidth}

\Xhline{3\arrayrulewidth}

\multirow{2}{*}{Unstructured} & \cite{guo2019reweighted} $^{A}$ & -- & 284 (67.6\%) & 194 (58.7\%) & 1x & 1x & -- & -- & -- & 88.5 & 0.0 \\
\cline{2-12}
\multirow{2}{*}{Pruning} & \cite{chen2020lottery} $^{*}$ $^{S}$ & -- & 206 (48.9\%) & 116 (35.1\%) & 1x & 1x & 83.1 & 89.5 & 92.9 & 87.8 & -0.63 \\
\cline{2-12}
 & \cite{sanh2020movement} $^{S}$ & -- & 100 (23.8\%) & 10 (3\%) & 1x & 1x & 79.0 & 89.3 & -- & 79.9 & -4.73 \\

\Xhline{3\arrayrulewidth}
Structured & \cite{lin2020pruning} $^{S}$ & -- & 255 (60.7\%) & 165 (50\%) & -- & -- & -- & 88.9 & 91.8 & -- & -1.0 \\
\cline{2-12}
Pruning & \cite{khetan2020schubert} $^{A}$ & -- & 164 (39.1\%) & 128 (38.8\%) & 2.93x$^{\ddagger}$ & $O$ & 83.4 & -- & 90.9 & 86.7 & -1.86 \\
% \cline{2-12}
% & \cite{sun2020contrastive} $^{A,S}$ $^{\dagger\dagger}$ $^{\dagger}$ & 255 (60.7\%) & 165 (50\%) & 1.94x & 1.73x & 83.5 & 89.1 & 93.6 & -- & -0.37 \\
% & \cite{lin2020pruning} & 45.0\% & 189 & 99 & -- & -- & -- & 87.8 & 88.4 & -- & -3.25 \\
% & \cite{fan2019reducing} $^{A,S}$ & 255 (60.7\%) & 165 (50\%) & 1.94x & 1.73x & 82.9 & -- & 92.5 & -- & -1.35 \\
\Xhline{3\arrayrulewidth}

% \multicolumn{3}{l}{Knowledge Distillation}  \\
% \Xhline{3\arrayrulewidth}
\multirow{2}{*}{KD from} & \cite{song2020lightpaff} $^{A,S}$ & V100 & 96 (22.8\%) & 36 (10.9\%) & 6.25x & 7.09x & -- & 88.6 & 92.9 & -- & -0.6 \\
\cline{2-12}
\multirow{2}{*}{Output Logits} & \cite{liu2019attentive}$^{\S}$ $^{S}$ & V100 & 101 (24.1\%) & 11 (3.3\%) & 10.7x & $O$ & 78.6 & 88.6 & 91.0 & -- & -3.03 \\
\cline{2-12}
 & \cite{chen2020adabert} $^{*}$ $^{A,S}$ & V100 & 31 (7.4\%) & 16 (4.8\%) & 19.5x$^{*}$ & -- & 81.6 & 88.7 & 91.8 & -- & -2.06 \\

\Xhline{3\arrayrulewidth}

% \multirow{2}{*}{KD-EO} & 60.5\% & 2x & 82.2 & 88.5 & 91.3 & 86.9 & 16.45 \\
% \cline{2-8}
%  & 1.6\% & -- & 71.0 & -- & 82.8 & -- & 7.23 \\
% \Xhline{3\arrayrulewidth}

KD from Attn. & \cite{wang2020minilm} $^{A}$ & P100 & 255 (60.7\%) & 165 (50\%) & 1.94x & 1.73x & 84.0 & 91.0 & 92.0 & -- & -0.1 \\

\Xhline{3\arrayrulewidth}


\multirow{3}{*}{Multiple KD} & \cite{sanh2019distilbert} $^{A}$ & CPU & 255 (60.7\%) & 165 (50\%) & 1.94x & 1.73x & 82.2 & 88.5 & 91.3 & 86.9 & -1.73 \\
\cline{2-12}
\multirow{3}{*}{combined} & \cite{sunmobilebert}$^{\S}$ $^{A}$ & Pixel & 97 (23.1\%) & 82 (24.8\%) & $C$ & $C$ & 83.3 & -- & 92.8 & 90.0 & -0.16 \\
% mobilebert - 5.52x on pixel phone
\cline{2-12}
 & \cite{jiao2019tinybert} $^{A,S}$ & K80 & 56 (13.3\%) & 21 (6.4\%) & 9.4x & $O$ & 82.5 & 89.2 & 92.6 & -- & -1.0\\
\cline{2-12}
 & \cite{zhao2019extreme} $^{A}$ & -- & 6.8 (1.6\%) & 5.9 (1.8\%) & 25.5x$^{\ddagger}$ & $O$ & 71.3 & -- & 82.2 & -- & -12.3 \\

\Xhline{3\arrayrulewidth}

Matrix & \cite{noach2020compressing} $^{S}$ & Titan V & 252 (60.6\%) & 162 (49.1\%) & 0.92x & 1.05x & 84.8 & 89.7 & 92.4 & -- & -0.13 \\
\cline{2-12}
Decomposition & \cite{cao2019} $^{S}$ & V100 & 420 (100\%) & 330 (100\%) & 3.14x & 3.55x & 82.6 & 90.3 & -- & 87.1 & -0.76 \\ 
% \cline{2-12}
%  & \cite{wang2020linformer} $^{\dagger}$ $^{A}$ & 420 (100\%) & 330 (100\%) & 1.6x & -- & -- & 90.5 & 93.2 & -- & +0.4 \\
\Xhline{3\arrayrulewidth}

Dynamic & \cite{xin2020deebert} $^{S}$ & P100 & 420 (100\%) & 330 (100\%) & 1.25x & $C$ & 83.9 & 89.2 & 93.4 & -- & -0.26 \\
\cline{2-12}
Speedup & \cite{goyalpower} $^{S}$ & K80 & 420 (100\%) & 330 (100\%) & 2.5x & $C$ & 83.8 & -- & 92.1 & -- & -1.1 \\
% \cline{2-12}
% & \cite{zhou2020bert} $^{S}$ & 420 (100\%) & 330 (100\%) & 1.62x & -- & 83.6 & -- & 92.0 & -- & -1.25 \\
\Xhline{3\arrayrulewidth}

Param. Sharing & \cite{lan2019albert} $^{A}$ & -- & 45 (10.7\%) & 29 (8.8\%) & 1.2x $^{\ddagger}$ & $C$ & 84.3 & 89.6 & 90.3 & 89.3 & -0.58 \\

\Xhline{3\arrayrulewidth}

Pruning & \cite{mao2020ladabert} $^{S}$ & -- & 168 (40.0\%) & 123 (37.3\%) & 1x & 1x & 83.5 & 88.9 & 92.8 & -- & -0.7 \\
% \cline{2-8}
%  & \cite{sanh2020movement} & 25.9\% & 1x & 80.2 & 89.3 & 82.4 & -- \\
\cline{2-12}
with KD & \cite{hou2020dynabert} $^{S}$ & K40 & 131 (31.2\%) & 41 (12.4\%) & 5.9x$^{\ddagger}$ & 8.7x$^{\ddagger}$ & 82.0 & 90.4 & 92.0 & -- & -0.96 \\

\Xhline{3\arrayrulewidth}

Quantization & \cite{zadeh2020gobo} $^{S}$ & CPU & 32 (7.6\%) & 13 (3.9\%) & 1.94x & 1.73x & 82.0 & -- & -- & -- & -2.6 \\
% \cline{2-8}
%  & \cite{sanh2020movement} & 25.9\% & 1x & 80.2 & 89.3 & 82.4 & -- \\
\cline{2-12}
with KD & \cite{sunmobilebert}$^{\S}$ $^{A}$ & Pixel & 24 (5.7\%) & 20 (6.1\%) & $C$ & $C$ & 83.3 & -- & 92.6 & 90.0 & -0.23 \\
% mobilebert quant pixel --  5.52x

\Xhline{3\arrayrulewidth}


Compound  & \cite{tambe2020edgebert} $^{S}$ & TX2 & 5.5 (1.3\%) & 3.8 (0.9\%) & 1.83x & -- & 84.4 & 89.8 & 88.5 & -- & -1.53 \\

\Xhline{3\arrayrulewidth}

\end{tabular}

% \footnotemark{For methods that allow varying model size for different tasks, we used the average to represent the model size and the speedup.}

% \footnotemark{$\Delta MS$ is the drop in model size, and $\Delta A$ is the drop in accuracy for the MNLI task.}
\caption{
Evaluation of various compression methods. 
$^{*}$ indicates models using task-specific sizes or speedups; average values are reported in such cases. 
% $^{\dagger}$ marks models trained using optimizations proposed by RoBERTa \cite{liu2019roberta}. 
$^{\S}$ represents models that use $\mathrm{BERT_{LARGE}}$ as the teacher model. 
% $^{\dagger\dagger}$ Teacher is Roberta. 
$^{\ddagger}$ shows the speedups that we calculated. 
\textcolor{red}{$C$ : Methods which have open source code, and I can calculate speedup. 
$O$ : Methods which have clearly defined final compressed models, and I can calculate speedup.}
}
\label{tab:evaluation_small}
\end{table*}

==> tables/table_arch.tex <==
\begin{table}[]
\footnotesize
\centering
%\vspace{-2mm}
\setlength\tabcolsep{2pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{\textbf{Component}} & \multirow{2}{*}{\textbf{DQ}} & \multicolumn{2}{c}{\textbf{PR}} & \multicolumn{3}{|c|}{\textbf{KD}} & \multicolumn{2}{|c|}{\textbf{AIC}} \\
\cline{3-9}
 & &\textbf{EP} & \textbf{SP} & \textbf{EO} & \textbf{OL} & \textbf{AM} & \textbf{PS} & \textbf{EMC} \\
\Xhline{3\arrayrulewidth}

Embedding Layer & $\checkmark$ & & & $\bigtriangleup$ & $\bigtriangleup$ & & & $\bigtriangleup$ \\
\hline
Self Attention & $\checkmark$ & $\checkmark$ & $\bigtriangleup$ & $\bigtriangleup$ & $\bigtriangleup$ & $\bigtriangleup$ & & \\
\hline
Feed Forward Network & $\checkmark$ & $\checkmark$ & & $\bigtriangleup$ & $\bigtriangleup$ & & & \\
\Xhline{3\arrayrulewidth}
Transformer & & & & $\bigtriangleup$ & $\bigtriangleup$ & & $\checkmark$ & \\
\Xhline{3\arrayrulewidth}
\end{tabular}

$\checkmark$ indicates the requirement of the original BERT training corpus. \\
$\bigtriangleup$ indicates the requirement of only task-specific datasets.
\caption{Compression methods and their corresponding target architectural components in BERT.}\label{tab:compression}
%\vspace{-4mm}
\end{table}


% Embed. layer & $\checkmark^{\ciao{1}}$ & & & & & & & $\checkmark^{\ciao{15}}$ & & \\
% \hline
% Self-Attn. & $\checkmark^{\ciao{2}}$ & $\checkmark^{\ciao{4}}$ & $\checkmark^{\ciao{6}}$ & $\checkmark^{\ciao{7}}$ & $\checkmark^{\ciao{10}}$ & $\checkmark^{\ciao{13}}$ & & & $\checkmark^{\ciao{16}}$ & \\
% \hline
% FFN & $\checkmark^{\ciao{3}}$ & $\checkmark^{\ciao{5}}$ & & $\checkmark^{\ciao{8}}$ & $\checkmark^{\ciao{11}}$ & & & & & \\
% \Xhline{2\arrayrulewidth}
% Transformer & & & & $\checkmark^{\ciao{9}}$ & $\checkmark^{\ciao{12}}$ & & $\checkmark^{\ciao{14}}$ & & & $\checkmark^{\ciao{17}}$ \\

==> tables/table_best_methods.tex <==
\begin{table*}
%\vspace{-3mm}
\footnotesize
%\vspace{-2mm}
\centering
\setlength\tabcolsep{4.5pt}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\Xhline{3\arrayrulewidth}
\textbf{Paper} & \textbf{Compression} & \textbf{Model} & \textbf{Speedup} & \multicolumn{4}{|c|}{\textbf{Accuracy/F1}} & \multirow{2}{*}{$\mathbold{\frac{\Delta MS}{\Delta A}}$$^\dagger$}\\
\cline{5-8}
 & \textbf{Method} & \textbf{Size} & & \textbf{MNLI} & \textbf{QQP} & \textbf{SST-2} & \textbf{SQD} & \\
\Xhline{3\arrayrulewidth}

$\mathrm{BERT}_{\mathrm{BASE}}$ & -- & 100\% & 1x & 84.6 & 89.2 & 93.5 & 88.5 & -- \\
\Xhline{3\arrayrulewidth}

\cite{shen2019q} & DQ & 15.3\% & -- & 83.9 & -- & 92.7 & 88.3 & 121 \\
\hline

\cite{zadeh2020gobo} & DQ & 10.2\% & -- & 83.7 & -- & -- & -- & 99.77 \\
\hline

\cite{wang2020minilm} & KD-AM & 60.5\% & 2x & 84.0 & 91.0 & 92.0 & -- & 65.83 \\
\hline

\cite{hou2020dynabert} & SP +KD-EO+OL & 37.5\% & -- & 83.6 & 91.2 & 92.8 & -- & 62.5 \\
\hline

\cite{mao2020ladabert} & EP + KD-EO+OL+AM & 40\% & -- & 83.5 & 88.9 & 92.8 & -- & 54.54\\
\hline

\cite{xu2020bert} & SP & 60.5\% & -- & 83.7 & 91.1 & 92.7 & -- & 43.88 \\
\hline

\cite{jiao2019tinybert} & KD-EO+OL+AM & 13.3\% & 9.4x & 82.5 & 89.2 & 92.6 & -- & 41.28 \\

\Xhline{3\arrayrulewidth}

\end{tabular}

\footnotemark{$\Delta MS$ is the drop in model size, and $\Delta A$ is the drop in accuracy for the MNLI task.}
\caption{A collection of current best performing compression methods in literature.}
\label{tab:best_methods}
%\vspace{-5mm}
\end{table*}

==> tables/table_eval.tex <==
\begin{table*}
\scriptsize
\caption{Evaluation comparison of various compression methods. OPT = Optimization by replacing layernorm with linear transformation and gelu with relu; PKD = Patient Knowledge Distillation; RPP = Reweighted Proximity Pruning; QAT = Quantization Aware Training; MP = Mixed Precision; SRA = Sentence Representation Approximation; BNN = Biattentive Neural Network; TS = Transfer Set. * For methods which provide varying size of models for different tasks, we have used the average to represent the model size and speedup}
\label{tab:evaluation}
\centering
\setlength\tabcolsep{0.9pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Paper}} & \textbf{Compression} & \multirow{2}{*}{\textbf{Model}} & \textbf{Model Size /} & \multicolumn{11}{|c|}{\textbf{Accuracy/F1}} \\
\cline{5-15}
 & \textbf{Method} & & \textbf{Speedup} & \textbf{MNLI-m/mm} & \textbf{QQP} & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{STS-B} & \textbf{MRPC} & \textbf{RTE} & \textbf{SQD1.1} & \textbf{SQD2.0} & \textbf{RACE} \\
\hline

\multirow{2}{*}{\cite{devlin2019bert}} & \multirow{2}{*}{--} & $\mathrm{BERT}_{\mathrm{BASE}}$ & 100\% / 1x & 84.6/83.4 & 89.2/71.2 & 90.5 & 93.5 & 52.1 & 87.1/85.8 & 88.9/84.8 & 66.4 & 88.5 & -- & -- \\
\cline{3-15}
 & & $\mathrm{BERT}_{\mathrm{LARGE}}$ & 309\% / 0.29x & 86.7/85.9 & 89.3/72.1 & 92.7 & 94.9 & 60.5 & 87.6/86.5 & 89.3/85.4 & 70.1 & 90.9 & 81.9 & --  \\
\hline

\multirow{2}{*}{\cite{lan2019albert}} & \multirow{2}{*}{\ciao{14}\ciao{15}} & $\mathrm{ALBERT}_{\mathrm{BASE}}$ & 11.1\% / -- & 81.6/-- & -- & -- & 90.3 & -- & -- & -- & -- & 89.3 & 80.0 & 64.0 \\
 \cline{3-15}
 & & $\mathrm{ALBERT}_{\mathrm{XXLARGE}}$ & 217\% / -- & 88.0/-- & -- & -- & 95.2 & -- & -- & -- & -- & 94.1 & 88.1 & 82.3 \\
\hline


\multirow{2}{*}{\cite{sunmobilebert}} & \multirow{2}{*}{\ciao{8}\ciao{13}(L)} & MobileBERT & 23.2\% / 2.36x & 84.3/83.4 & 88.3/70.5 & 91.6 & 92.6 & 51.1 & 86.2/84.8 & 88.8/84.5 & 70.4 & 90.2 & 79.2 & -- \\
\cline{3-15}
 & & MobileBERT w/ OPT & 23.2\% / 4x & 83.3/82.6 & 88.0/70.2 & 90.6 & 92.8 & 50.5 & 84.4/82.7 & 88.8/84.6 & 68.2 & 90.3 & 80.2 & -- \\
\hline

\multirow{3}{*}{\cite{sun2019patient}} & \multirow{3}{*}{\ciao{9}\ciao{12}(L)} & $\mathrm{BERT}_{\mathrm{BASE}}$ & 100\% / 1x & 83.7/82.2 & 89.0/70.9 & 90.4 & 94.3 & -- & -- & 89.2/85.2 & 69.1 & -- & -- & 65.3 \\
\cline{3-15}
 & & $\mathrm{BERT_{6}-PKD}$ & 60.5\% / 1.94x & 81.5/81.0 & 88.9/70.7 & 89.0 & 92.0 & -- & -- & 85.0/79.9 & 65.5 & -- & -- & 60.34 \\
\cline{3-15}
 & & $\mathrm{BERT_{3}-PKD}$ & 41.9\% / 3.73x & 76.7/76.3 & 87.8/68.1 & 84.7 & 87.5 & -- & -- & 80.7/72.5 & 58.2 & -- & -- & -- \\
\hline

\multirow{2}{*}{\cite{jiao2019tinybert}} & \ciao{7}\ciao{8}\ciao{10} & $\mathrm{BERT}_{\mathrm{BASE}}$ & 100\% / 1x & 83.9/83.4 & --/71.1 & 90.9 & 93.4 & 52.8 & --/85.2 & 87.5/-- & 67.0 & -- & -- & --  \\
\cline{3-15}
 & \ciao{11}\ciao{13}(B) & $\mathrm{TinyBERT}_{\mathrm{}}$ & 13.3\% / 9.4x & 82.5/81.8 & 89.2/71.3 & 87.7 & 92.6 & 43.3 & 81.2/79.9 & 86.4/81.2 & 62.9 & -- & -- & --  \\
\hline

\multirow{2}{*}{\cite{sanh2019distilbert}} & \multirow{2}{*}{\ciao{9}\ciao{12}(B)} & $\mathrm{RoBERTa}_{\mathrm{BASE}}$ & 100\% / 1x & --/84.3 & 89.5/-- & 89.3 & 91.7 & 48.9 & 91.2/-- & 88.6/-- & 71.3 & 88.5 & -- & --  \\
\cline{3-15}
 & & $\mathrm{DistilBERT}_{\mathrm{}}$ & 60.5\% / 1.63x & --/81.8 & 89.2/-- & 90.2 & 92.7 & 49.1 & 90.7/-- & 90.2/-- & 62.9 & 86.9 & -- & -- \\
\hline

\multirow{2}{*}{\cite{zhao2019extreme}} & \ciao{7}\ciao{8}\ciao{10} & $\mathrm{BERT}_{\mathrm{BASE}}$ & 100\% / 1x & 84.0/82.8 & -- & -- & 93.5 & -- & -- & 88.5/84.3 & -- & -- & -- & -- \\
\cline{3-15}
 & \ciao{11}\ciao{15}(B) & $\mathrm{BERT}_{\mathrm{EXTREME}}$ & 1.6\% / -- & 71.0/70.8 & -- & -- & 82.8 & -- & -- & 79.3/68.6 & -- & -- & -- & -- \\
\hline

\multirow{3}{*}{\cite{guo2019reweighted}} & \multirow{3}{*}{\ciao{4}\ciao{5}} & $\mathrm{BERT}_{\mathrm{BASE}}$ & 100\% / 1x & 86.1/85.9 & 91.2/-- & 91.3 & 93.2 & 81.8 & -- & 89.3/-- & 70.1 & 90.9 & 81.9 & -- \\
\cline{3-15}
 & & $\mathrm{BERT}_{\mathrm{RPP}}$ & 53.6\% / -- & 86.1/85.7 & 91.2/-- & 92.3 & 92.4 & 82.8 & -- & 88.1/-- & 70.1 & 90.2 & 81.3 & -- \\
 \cline{3-15}
 & & $\mathrm{BERT}_{\mathrm{RPP\_Ext}}$ & 30.9\% / -- & 81.4/81.8 & 89.2/-- & 88.0 & 90.5 & 79.3 & -- & 81.9/-- & 67.5 & 81.7 & 80.7 & -- \\
\hline

\multirow{2}{*}{\cite{zafrir2019q8bert}} & \multirow{2}{*}{\ciao{1}\ciao{2}\ciao{3}} & $\mathrm{BERT}_{\mathrm{BASE}}$ & 100\% / 1x & -- & 87.8/-- & 90.3 & 92.3 & 58.5 & 89.6/-- & 90.0/-- & 69.7 & 87.7 & -- & --  \\
\cline{3-15}
 & & $\mathrm{Q8BERT}_{\mathrm{QAT}}$ & 25\% / -- & -- & 87.9/-- & 90.6 & 92.2 & 58.5 & 89.0/-- & 89.5/-- & 68.8 & 88.5 & -- & --  \\
\hline

\multirow{3}{*}{\cite{shen2019q}} & \multirow{3}{*}{\ciao{1}\ciao{2}\ciao{3}} & $\mathrm{BERT}_{\mathrm{BASE}}$ & 100\% / 1x & 84.0/84.4 & -- & -- & 93.0 & -- & -- & -- & -- & 88.7 & -- & --  \\
\cline{3-15}
 & & $\mathrm{BERT}_{\mathrm{2/4 MP}}$ & 12.8\% / -- & 83.5/83.6 & -- & -- & 92.5 & -- & -- & -- & -- & 87.5 & -- & --  \\
\cline{3-15}
 & & $\mathrm{BERT}_{\mathrm{2/3 MP}}$ & 11.5\% / -- & 81.7/82.3 & -- & -- & 92.1 & -- & -- & -- & -- & 87.0 & -- & --  \\
\hline

\cite{tang2019distilling} & \ciao{12}\ciao{17}(L) & $\mathrm{BiLSTM}_{\mathrm{SOFT}}$ & 9.2\% / -- & 73.0/72.6 & 88.1/68.2 & -- & 90.7 & -- & -- & -- & -- & -- & -- & --  \\
\hline

\cite{bowentowards} & \ciao{9}\ciao{17}(B) & $\mathrm{BiLSTM}_{\mathrm{SRA}}$ & 4.4\% / 17.7x & 72.6/72.5 & 86.2/64.4 & -- & 89.8 & -- & -- & 83.1/75.1 & -- & -- & -- & -- \\
\hline

\cite{liu2019attentive} & \ciao{12}\ciao{17} (L) & $\mathrm{BiLSTM}_{\mathrm{BNN}}$ & 11.7\% / -- & 78.6/78.4 & 88.6/70.7 & 85.4 & 91.0 & -- & 80.9/80.9 & 85.4/79.7 & 67.3 & -- & -- & -- \\
\hline

\cite{tang2019natural} & \ciao{12}\ciao{17} (L) & $\mathrm{BiLSTM}_{\mathrm{TS}}$ & 9.2\% / -- & -- & -- & -- & 92.7 & 40.0 & 82.1/80.7 & 85.5/80.2 & -- & -- & -- & -- \\
\hline

\cite{turc2019well} & \ciao{10}\ciao{11}\ciao{12}(B) & $\mathrm{BERT_{6}-PD}$ & 60.5\% / -- & 82.8/82.2 & 88.9/70.4 & 88.9 & 91.8 & -- & -- & 86.8/81.7 & 65.3 & -- & -- & -- \\
\hline

\multirow{2}{*}{\cite{cao2019}} & \multirow{2}{*}{\ciao{7}\ciao{10}\ciao{16}(B)} & $\mathrm{BERT}_{\mathrm{BASE}}$ & 100\% / 1x & 84.4/-- & 90.5/-- & -- & -- & -- & -- & -- & -- & 88.5 & -- & 66.3 \\
\cline{3-15}
 & & $\mathrm{Decomp BERT}_{\mathrm{BASE}}$ & 100\% / 2.7x* & 82.6/-- & 90.3/-- & -- & -- & -- & -- & -- & -- & 87.1 & -- & 64.5 \\
\hline

\multirow{2}{*}{\cite{chen2020adabert}} & \multirow{2}{*}{\ciao{9}\ciao{12}\ciao{17}(B)} & $\mathrm{BERT}_{\mathrm{BASE}}$ & 100\% / 1x & 84.8/-- & --/71.1 & 90.4 & 93.3 & -- & -- & 88.7/-- & 66.1 & -- & -- & --  \\
\cline{3-15}
 & & AdaBERT & 7.3\%* / 21x* & 81.6/-- & --/70.7 & 86.8 & 91.8 & -- & -- & 85.1/-- & 64.4 & -- & -- & -- \\
\hline
% \hline

% \cite{michel2019sixteen} & Att. head Pruning & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \hline

% -- & BiLSTM & BASE & 11.9\% / -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --  \\
% \hline

\end{tabular}
\end{table*}
